On Two Distinct Sources of Nonidentifiability in Latent Position Random Graph Models

Two separate and distinct sources of nonidentifiability arise naturally in the context of latent position random graph models, though neither are unique to this setting. In this paper we define and examine these two nonidentifiabilities, dubbed subspace nonidentifiability and model-based nonidentifiability, in the context of random graph inference. We give examples where each type of nonidentifiability comes into play, and we show how in certain settings one need worry about one or the other type of nonidentifiability. Then, we characterize the limit for model-based nonidentifiability both with and without subspace nonidentifiability. We further obtain additional limiting results for covariances and $U$-statistics of stochastic block models and generalized random dot product graphs.

==> formatting/jmlr/jmlr_title_abstract.tex <==
\title{On Two Distinct Sources of Nonidentifiability in Latent Position Random Graph Models}
\date{}
\author{\name Joshua Agterberg \email jagterberg@jhu.edu \\
       \addr Department of Applied Mathematics and Statistics\\
       Johns Hopkins University\
       Baltimore, MD  21211, USA 
       \AND
       \name Minh Tang
\email mtang8@ncsu.edu \\
\addr Department of Statistics \\
North Carolina State University
       \AND
       \name Carey E. Priebe \email cep@jhu.edu  \\
       \addr Department of Applied Mathematics and Statistics\\
       Johns Hopkins University\
       Baltimore, MD 21211, USA }

\editor{}
\maketitle

\begin{abstract}%   <- trailing '%' for backward compatibility of .sty file
Two separate and distinct sources of nonidentifiability 
arise naturally in the context of latent position random graph models,
though neither are unique to this setting.
In this paper we define and examine these two nonidentifiabilities,
dubbed {\it subspace nonidentifiability} and {\it model-based nonidentifiability},
in the context of random graph inference.  We give examples where each type of nonidentifiability comes into play, and we show how in certain settings one need worry about one or the other type of nonidentifiability. Then, we characterize the limit for model-based nonidentifiability both with and without subspace nonidentifiability.  We further obtain additional limiting results for covariances and $U$-statistics of stochastic block models and generalized random dot product graphs.
\end{abstract}

\begin{keywords}
  Random Graphs, Stochastic Blockmodel, Identifiability
\end{keywords}

==> formatting/jmlr/preamble_jmlr.tex <==
%\usepackage{amsmath,amsfonts,amsthm,amssymb,mathrsfs}
%\usepackage{natbib} 
%\usepackage{hyperref}
\usepackage{mathtools}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argsup}{arg\,sup}
\newcommand\eqd {\overset{\mathrm{d}}{=}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\N}{\mathbb{N}} \newcommand{\Z}{\mathbb{Z}} \newcommand{\Q}{\mathbb{Q}} \newcommand{\R}{\mathbb{R}}
\newcommand{\s}{^*}
\renewcommand{\t}{^{\top}}
\newcommand{\inv}{^{-1}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\p}{\mathbb{P}}
\newcommand{\ipq}{\mathbf{I}_{p,q}}
%\newtheorem*{proposition}{Proposition}
%\newtheorem*{theorem}{Theorem}
%\newtheorem*{corollary}{Corollary}
%\newtheorem*{lemma}{Lemma}
%\theoremstyle{definition} 
%\newtheorem*{definition}{Definition}
%\newtheorem*{remark}{Remark}
%\newtheorem*{assumption}{Assumption}

\jmlrheading{1}{2020}{}{}{}{}{J. Agterberg, M. Tang, C.E. Priebe}


\ShortHeadings{Two Sources of Nonidentifiability}{Agterberg, Tang, and Priebe}
\firstpageno{1}

%\jmlrheading{1}{2000}{1-48}{4/00}{10/00}{author list}

